Classifying Constructive Comments

We introduce the Constructive Comments Corpus (C3), comprised of 12,000 annotated news comments, intended to help build new tools for online communities to improve the quality of their discussions. We define constructive comments as high-quality comments that make a contribution to the conversation. We explain the crowd worker annotation scheme and define a taxonomy of sub-characteristics of constructiveness. The quality of the annotation scheme and the resulting dataset is evaluated using measurements of inter-annotator agreement, expert assessment of a sample, and by the constructiveness sub-characteristics, which we show provide a proxy for the general constructiveness concept. We provide models for constructiveness trained on C3 using both feature-based and a variety of deep learning approaches and demonstrate that these models capture general rather than topic- or domain-specific characteristics of constructiveness, through domain adaptation experiments. We examine the role that length plays in our models, as comment length could be easily gamed if models depend heavily upon this feature. By examining the errors made by each model and their distribution by length, we show that the best performing models are less correlated with comment length.The constructiveness corpus and our experiments pave the way for a moderation tool focused on promoting comments that make a contribution, rather than only filtering out undesirable content.

==> tables/LB-CTC_CTC_experiments.tex <==
 \begin{table}[ht]
    \centering
    \begin{tabular}{llrr}
    \toprule
    \textbf{Train}    &
    \textbf{Model}  &
    \textbf{F1 on \CTC}  &   \textbf{F1 on LB-\CTC}\\
    &   &   (test portion)  &   (test portion)\\
    \midrule
    \multirow{3}{*}{\CTC}   & SVM (all - length)                         &   -     &   -\\
    & biLSTM    &   0.93    &   0.56\\
    & CNN    &   0.88    &   0.56\\
    \midrule
    \multirow{3}{*}{LB-\CTC}   & SVM (all - length)                         &   -    &   -\\
    & biLSTM    &   0.70    &   0.67\\
    & CNN    &   0.50   &   0.55\\    
    \bottomrule 
    \end{tabular}
    \caption{Results of the length experiments.}
    \label{tab:length_experiments}
\end{table}

==> tables/dataset_results_tbl.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lrr}
    \toprule
    \textbf{Dataset}    & \textbf{Size}    &  \textbf{CV}\\
    \midrule
    \CTC  &   10,762 &   0.96\\
    \smCTC  & 1,035 &   0.86\\
%    \CTC + \smCTC  &  11,797 &   0.95\\
    \NYT + \YNACC  & 30,325    &    0.89\\
%    \CTC + \NYT + \YNACC & 41,087 &   0.91\\    
%    \CTC(NC) + \NYT & 9,712 &   0.94\\
    \bottomrule
    \end{tabular}
    \caption{Mean F1 scores of 10-fold cross-validation experiments on different datasets. The experiments were run with all features from Table \ref{tab:constructiveness_feats}.}
    \label{tab:datasets_results}
\end{table}


==> tables/datasets_stats_tbl.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{llrrr}
    \toprule
    \textbf{Dataset}    &  \textbf{Label}    & \textbf{Size}  &   \textbf{AvgLen}    &   \textbf{AvgSents}\\
    \midrule
    \multirow{2}{*}{\CTC}  & C &   5,906   &   117.4   &   6.8\\
                        &   NC & 4,856    &   21.4   &   2.0\\
    \midrule
    \multirow{2}{*}{\smCTC}  & C &  551   &   97.1   &   5.8\\
                        &  NC & 484   &   22.8   &   2.1\\
    \midrule
    \multirow{1}{*}{\NYT}  & C &  15,147   &   131.7   &   7.4\\
    \midrule
    \multirow{1}{*}{\YNACC}  &  NC & 15,178  &   41.1   &   3.4\\

    %\smCTC  & 551  & 484\\     
    %\NYT    & 15,147    &   0   \\
    %\YNACC  &  0    &   15,178\\ 
    \bottomrule \\
    \end{tabular}
    \caption{Distribution of constructive and non-constructive comments in different datasets. C=constructive. NC=non-constructive. AvgLen=average length in words. AvgSents=average number of sentences.}
    \label{tab:datasets}
\end{table}

==> tables/length_experiments.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lrr}
    \toprule
    \textbf{Model}    &  \textbf{Train\CTC}  &   \textbf{Train\NYT}\\
    \midrule
    Lexical  & 0.57 & 0.62\\
    Part-of-speech  & 0.58  & 0.59\\
    Length  & 0.53  &  0.61\\
    Argumentation  & 0.51  & 0.51\\
    Named-entity & 0.51  & 0.52\\    
    Text quality & \textbf{0.59}  & 0.61\\
    Content quality &  \textbf{0.59} & 0.61\\
    Aggressiveness & 0.54  & 0.56\\
    Toxicity & 0.53  & 0.57\\
    All features & 0.56  & \textbf{0.63}\\
    biLSTM  & 0.57  &   0.57\\
    CNN  & 0.55   & 0.58\\ 
    \bottomrule 
    \end{tabular}
    \caption{Results on the length-balanced subset of \CTC(LB-\CTC), containing 587 constructive and 587 non-constructive comments.}
    \label{tab:length_experiments}
\end{table}

==> tables/top_lexical_pos_feats_tab.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lll|lll}
    \toprule
    \multicolumn{3}{c}{Constructive}    & \multicolumn{3}{c}{Non-constructive}\\
    ngram   &   tfidf   &   pos &   ngram   &   tfidf   &   pos \\
\midrule
religious   &   people  &   punct det   &   &   &  \\
currently   &  government   &  punct adv    &   &   &   \\
population   &  years   &  punct adp   &   &   &   \\
said    &   canada  &   punct cconj   &   &   &   \\
true    &   world   &   punct verb  &   &   &   \\
workers &   country &   punct num  &   &   &   \\
citizens    &   time    &   punct propn  &   &   &   \\
country   &   public  &   punct pron  &   &   &   \\
likely &   way &   punct noun  &   &   &   \\
opposition  &   canadian    &   punct adj  &   &   &  \\

    \bottomrule
    \end{tabular}
    \caption{Top 10 ngrams, tfidf features, and pos sequences}
    \label{tab:top_lexical_feats}
\end{table}

